LLM-Powered Multi-Agent System for Automated Crypto Portfolio Management

Cryptocurrency portfolio management requires the fusion of heterogeneous multi-modal signals, including structured price and on-chain time series, unstructured news text, and technical indicators, under high-volatility and real-time constraints. While deep learning approaches show predictive capability, their opacity limits practical adoption, and single large language model (LLM) agents struggle to process the breadth of modality-specific inputs needed for robust decision-making. We propose a multi-agent system (MAS) framework in which three modality-specialised agents, a Crypto Agent for market dynamics, a News Agent for weekly news sentiment, and a Trading Agent for signal fusion and portfolio execution, decompose the task across three communication architectures: hierarchical, collaborative, and debate. We evaluate four capability configurations: zero-shot, chain-of-thought (CoT), retrieval-augmented generation (RAG), and skill-augmented. In a 52-week backtest over calendar year 2025 across the top 15 L1 blockchain native cryptocurrencies by market capitalisation as of January 2025, the best configuration, Hierarchical (Skill), achieves a cumulative return of 133.52% and a Sharpe ratio of 1.502, outperforming single-agent variants, passive benchmarks, and deep learning baselines. An ablation study identifies the Crypto Agent as the most critical component, with its removal reducing cumulative return by 42.57 percentage points. A cross-model comparison further shows that MAS outperforms the single-agent baseline under GPT-4o, GPT-5, and Claude Sonnet 4.5, suggesting that the benefit of multi-agent coordination is model-agnostic. Unlike black-box deep learning models, every portfolio decision is traceable to explicit agent reasoning, offering an interpretable and effective approach to multi-modal cryptocurrency portfolio management.

==> Prompts/crypto_explain.tex <==
\begin{prompt}[label={crypto_explain},nameref={explain}]{Crypto Factor Analyst.}
Learn the following cryptocurrency investment knowledge. Using this knowledge, explain the predicted price trend of \textcolor{blue}{\{\textit{target crypto}\}} for the upcoming week based on the provided information. The data for the top 30 cryptocurrencies, including \textcolor{blue}{\{\textit{target crypto}\}}, have been categorized into Very High, High, Medium, Low, and Very Low. Their respective predicted price trend has been categorized into Rise or Fall.


Knowledge: \textcolor{blue}{\{\textit{literature}\}}
(End of knowledge)


Information: \textcolor{blue}{\{\textit{factors}\}}
(End of information)


Price trend: \textcolor{blue}{\{\textit{future price trend}\}}
(End of price trend)
\end{prompt}

==> Prompts/crypto_prompt.tex <==
\begin{prompt}[label={crypto_prompt},nameref={crypto_prompt}]{Crypto Agent.}
Week: \textcolor{blue}{\{\textit{ISO week}\}}

Asset market data:
\textcolor{blue}{\{\textit{JSON array — per-asset close, volume, market\_cap for the last 30 days}\}}

Analyse each asset and return the JSON signal array.
\end{prompt}


==> Prompts/exp_instruc.tex <==
\begin{instruc}[label={exp_instruc},nameref={exp_instruc}]{Explanation Team.}
You are a professional cryptocurrency analyst, specializing in explaining the predicted {target} based on the provided knowledge and information. You should internalize the provided knowledge to generate a comprehensive explanation without explicitly referring to the literature. Your output should be in a single paragraph.
\end{instruc}

==> Prompts/ft.tex <==
\begin{prompt}[label={ft},nameref={ft}]{Fine-Tuning Market and Crypto Team.}
\textbf{User}: 

Analyze the following information of {crypto} to determine its \
{target} in a week. Please respond with Rise or Fall and provide your reasoning for the \
prediction.:

\textcolor{blue}{\{\textit{info}\}}
(End of information)

\textbf{Assistant}:

\textcolor{blue}{\{``Price trend"/``Market trend"\}}: \textcolor{blue}{\{\textit{trend}\}}

Explanation: \textcolor{blue}{\{\textit{expanation}\}}

\end{prompt}

==> Prompts/ft_instruc.tex <==
\begin{instruc}[label={ft_instruc},nameref={ft_instruc}]{Fine-Tuning Market and Crypto Team.}
You are a professional cryptocurrency analyst, specializing in predicting next week's \textcolor{blue}{\{``price trend of a cryptocurrency"/``market trend"\}} based on the provided information. Your output should be in the form of:\\
{Target}: (predicted {target})\\
Explanation: (your explanation)
\end{instruc}

==> Prompts/mkt_explain.tex <==
\begin{prompt}[label={mkt_explain},nameref={explain}]{Market Factor Analyst.}
Learn the following cryptocurrency investment knowledge. Using this knowledge, explain the predicted {target} for the upcoming week based on the provided information. The market factors have been categorized into Very High, High, Medium, Low, and Very Low using the first two years of data. The predicted market return has been categorized into Rise or Fall.

Knowledge: \textcolor{blue}{\{\textit{literature}\}}
(End of knowledge)

Information: \textcolor{blue}{\{\textit{factors/news}\}}
(End of information)

Market trend: \textcolor{blue}{\{\textit{future market trend}\}}
(End of market trend)
\end{prompt}

==> Prompts/news_explain.tex <==
\begin{prompt}[label={news_explain},nameref={explain}]{News Analyst.}
Learn the following cryptocurrency investment knowledge. Using this knowledge, explain the predicted {target} for the upcoming week on the provided news headlines. The predicted market return has been categorized into Rise or Fall.

Knowledge: \textcolor{blue}{\{\textit{literature}\}}
(End of knowledge)

Information: \textcolor{blue}{\{\textit{factors/news}\}}
(End of information)

Market trend: \textcolor{blue}{\{\textit{future market trend}\}}
(End of market trend)
\end{prompt}

==> Prompts/news_instruc.tex <==
\begin{instruc}[label={news_instruc},nameref={news_instruc}]{News Agent.}
You are the News Agent in a multi-agent cryptocurrency portfolio management system.

Your role is to read a set of Cointelegraph news articles from a single week and: (1) assess the overall market sentiment for the cryptocurrency market, and (2) extract coin-specific signals where articles mention specific cryptocurrencies. Each article is provided as a \textbf{title}, \textbf{published\_at} (UTC ISO timestamp), and \textbf{text} (article body).

Produce a JSON object with:
\begin{itemize}[leftmargin=10pt]
    \item \texttt{"overall\_sentiment"} — float in $[-1.0,\,1.0]$ \enspace ($-1=$ very bearish,\; $+1=$ very bullish)
    \item \texttt{"overall\_rationale"} — one-sentence summary of the news environment
    \item \texttt{"coin\_signals"} — array of objects, one per mentioned coin:
    \begin{itemize}[leftmargin=10pt]
        \item \texttt{"symbol"} — ticker from the universe (BTC, ETH, BNB, \ldots)
        \item \texttt{"signal"} — float in $[-1.0,\,1.0]$
        \item \texttt{"confidence"} — float in $[0.0,\,1.0]$
        \item \texttt{"rationale"} — one-sentence explanation
    \end{itemize}
\end{itemize}
Only include coins explicitly mentioned in the articles. Return ONLY valid JSON, no prose outside the JSON.
\end{instruc}


==> Prompts/news_prompt.tex <==
\begin{prompt}[label={news_prompt},nameref={news_prompt}]{News Agent.}
Week: \textcolor{blue}{\{\textit{ISO week}\}}

News articles (\textcolor{blue}{\{\textit{N}\}} total):
\textcolor{blue}{\{\textit{JSON array — per-article title, published\_at, text (truncated to 800 chars)}\}}

Analyse the news and return the JSON sentiment object.
\end{prompt}


==> Prompts/pred.tex <==
\begin{prompt}[label={pred},nameref={pred}]{Market and Crypto Team Prediction.}
Analyze the following \textcolor{blue}{\{``cryptocurrency"/"market"\}} information to determine the strength of the \textcolor{blue}{\{``price trend of a cryptocurrency"/``market trend"\}} in a week. Please respond with Rise or Fall and provide your reasoning for the prediction.

Information: \textcolor{blue}{\{\textit{factors/news/charts}\}}
(End of information)
\end{prompt}

==> Prompts/pred_instruc.tex <==
\begin{instruc}[label={pred_instruc},nameref={pred_instruc}]{Market and Crypto Team Prediction.}
You are a professional cryptocurrency analyst, specializing in predicting next week's \textcolor{blue}{\{``price trend of a cryptocurrency"/``market trend"\}} based on the provided candlestick chart. Your output should be in the form of:

\textcolor{blue}{\{``Price trend"/``Market trend"\}}: (predicted {target})

Explanation: (your explanation)
\end{instruc}

==> Prompts/rag_instruc.tex <==
\begin{instruc}[label={rag_instruc},nameref={rag_instruc}]{RAG Augmentation Addendum (appended to Crypto Agent system instruction).}
You will also receive historical analogues for each asset — past weeks with a similar price, volume, and market-capitalisation profile — retrieved by cosine similarity over an 11-dimensional scale-invariant feature vector of percentage changes (6 price-return horizons, 3 volume-change horizons, 2 market-cap-change horizons). Only entries strictly before the current week are eligible for retrieval. For each asset, the top-$K=3$ most similar past weeks are provided along with their realised next-week returns.

Use these historical precedents as additional empirical calibration when assessing the direction and strength of each asset's signal.
\end{instruc}


==> Prompts/skill_instruc.tex <==
\begin{instruc}[label={skill_instruc},nameref={skill_instruc}]{Skill Augmentation Addendum (appended to Crypto Agent system instruction).}
You will also receive pre-computed technical indicator values for each asset, derived from the same daily close price data. Indicators and interpretation rules:

\begin{itemize}[leftmargin=10pt]
    \item \textbf{SMA\_7} — 7-day simple moving average of closing price. Rule: close $>$ SMA\_7 $\rightarrow$ bullish (price above short-term trend); close $<$ SMA\_7 $\rightarrow$ bearish.
    \item \textbf{SMA\_30} — 30-day simple moving average. Rule: SMA\_7 $>$ SMA\_30 $\rightarrow$ bullish (golden cross); SMA\_7 $<$ SMA\_30 $\rightarrow$ bearish.
    \item \textbf{MACD\_hist} — MACD histogram $= (\text{EMA}_{12} - \text{EMA}_{26}) - \text{EMA}_9(\text{EMA}_{12} - \text{EMA}_{26})$. Rule: MACD\_hist $> 0$ $\rightarrow$ bullish (upward momentum); MACD\_hist $< 0$ $\rightarrow$ bearish.
    \item \textbf{BB\_lower} — Bollinger Band lower band $= \text{SMA}(20) - 2\,\sigma_{20}$. Rule: close $<$ BB\_lower $\rightarrow$ bullish (oversold, mean-reversion signal).
\end{itemize}

Use the count of bullish indicators $b \in \{0,1,2,3,4\}$ as composite signal strength: $b=4 \rightarrow$ strong buy; $b=0 \rightarrow$ strong sell; $b \in \{2,3\} \rightarrow$ moderate buy; $b=1 \rightarrow$ moderate sell.
\end{instruc}


==> Prompts/trading_prompt.tex <==
\begin{prompt}[label={trading_prompt},nameref={trading_prompt}]{Trading Agent.}
Week: \textcolor{blue}{\{\textit{ISO week}\}}

\textbf{overall\_news\_sentiment}: \textcolor{blue}{\{\textit{float in} $[-1,1]$\}}\\
\textbf{overall\_news\_rationale}: \textcolor{blue}{\{\textit{one-sentence market summary}\}}

\textbf{asset\_signals}:
\textcolor{blue}{\{\textit{JSON array — per-asset crypto signal, confidence, rationale, news signal, news confidence}\}}

\textbf{portfolio}:
\textcolor{blue}{\{\textit{JSON object — cash, per-asset value\_usd, cost\_basis\_usd, pnl\_usd, pnl\_pct, total\_value, total\_pnl\_usd, total\_pnl\_pct}\}}

Determine trading actions for all assets and return the JSON array.
\end{prompt}


==> Prompts/vision_explain.tex <==
\begin{prompt}[label={vision_explain},nameref={explain}]{Technical Analyst.}
\textbf{Text}: 

Learn the following cryptocurrency investment knowledge. Using this knowledge, explain the predicted price trend of \textcolor{blue}{\{\textit{target crypto}\}} for the upcoming week based on the provided candlestick chart. The chart includes candlesticks that depict daily opening, high, low, and closing prices. It then overlays a 30-day moving average closing price. The bottom of the chart shows daily trading volume.

Knowledge: \textcolor{blue}{\{\textit{literature}\}}
(End of knowledge)

Price trend: \textcolor{blue}{\{\textit{future price trend}\}}
(End of price trend)

\textbf{Image URL}: \textcolor{blue}{\{\textit{URL}\}}
\end{prompt}
